Sensitivity of Single-Pulse Radar Detection to Aircraft Pose Uncertainties

Mission planners for aircraft that operate in radar detection environments are often concerned the probability of detection. The probability of detection is a nonlinear function of the aircraft pose and radar position. Current path planning techniques for this application assume that the aircraft pose is deterministic. In practice, however, the aircraft pose is estimated using a navigation filter and therefore contains uncertainty. The uncertainty in the aircraft pose induces uncertainty in the probability of detection, but this phenomenon is generally not considered when path planning. This paper provides a method for combining aircraft pose uncertainty with single-pulse radar detection models to aid mission planning efforts. The method linearizes the expression for the probability of detection and three radar cross section models. The linearized models are then used to determine the variability of the probability of detection induced by uncertainty in the aircraft pose. The results of this paper validate the linearization using Monte Carlo analysis and explore the sensitivity of the probability of detection to aircraft pose uncertainty.

==> sections/Introduction.tex <==
\revisionD{
Manned and unmanned aircraft are often tasked with operating under threat of detection from ground-based radar systems. 
Mission planners must plan paths that maintain the probability of detection below mission-specified levels. Example missions in such environments include reconnaissance \cite{Ceccarelli_micro_uav}, radar counter-measure deployment \cite{larson_path_nodate,xiao-wei_path_2010}, and combat operations \cite{kabamba_optimal_2012}. A number of factors contribute to the probability of detection. The factors include the aircraft pose (i.e. position and orientation), intelligence about the radar systems, and the physical limitations of the aircraft (e.g. maneuverability, fuel usage).

A common assumption when modeling the detection probability is that the aircraft pose along the planned path is deterministic and known \cite{mcfarland_motion_1999,bortoff_path_2000,chandler_uav_2000,pachter_optimal_2001,moore_radar_2002,jun_path_2003,larson_path_nodate,kabamba_optimal_2012,xiao-wei_path_2010}. In practice, uncertainties in the aircraft pose come from a variety of sources. 
First, disturbances arise due to physical limitations and environmental factors (e.g. wind). 
Second, the inertial navigation system on the UAV estimates the pose of the aircraft using noisy and biased sensors \cite{savage_strapdown_2000, farrell_aided_2008, grewal_global_2020}.
Considering uncertainty in the aircraft pose is particularly important for regions where global position measurements may be contested, degraded, or denied.
}
In such regions, the aircraft pose uncertainties grow quickly and, as this paper demonstrates, become a significant source of variability in the probability of detection. 

This paper develops a framework for incorporating aircraft pose uncertainty in the calculation of the probability of detection for a single-pulse radar model. The resulting probability of detection is represented by a Gaussian distributed random variable with a mean and variance. A mission planner could use this information in path planning \cite{bry2011rapidly,blackmore_chance-constrained_2011}, error budget analysis \cite{maybeck_stochastic_1994,farrell_aided_2008,christensen2021closedloop}, or aircraft system design.

%\revision{
\revisionD{
The objective of the single-pulse radar model is to determine the instantaneous probability of detection given radar parameters, radar position, and the pose of the detected aircraft.
Marcum \cite{marcum_statistical_1960} expresses target detection as a probability using a nonlinear function of the radar parameters, target radar cross section (RCS), and range to target.
}
Swerling \cite{swerling_probability_1954} extends the work by Marcum to include fluctuating targets and multiple-pulse detection models.  

Mahafza \cite{mahafza_matlab_2003} extends the work by Marcum and Swerling to include considerations for modeling modern radar systems and provide expressions for common RCS models as a function of the aircraft pose relative to the radar. 
\revisionD{  
This work uses the probability of detection expressions and the constant and ellipsoid RCS models from Mahafza.
}
In addition, this work introduces the multi-lobed simple spikeball RCS model.

\revisionD{
Current path planning methods use a variety of radar models to evaluate the detection risk along candidate paths.
These models include proxies for the probability of detection to simplify the computation for the path planning algorithm.
Some proxies include integrated inverse range models \cite{bortoff_path_2000,chandler_uav_2000,pachter_optimal_2001,larson_path_nodate,xiao-wei_path_2010}, peak/aggregate RCS \cite{moore_radar_2002}, radar range equation \cite{mcfarland_motion_1999}, and a logistic function approximation with consolidated radar parameters \cite{kabamba_optimal_2012}. 
With the exception of \cite{kabamba_optimal_2012}, these methods do not attempt to quantify the probability of detection which is necessary for the mission planning scenario introduced above.
Futhermore, none of these approaches, including those presented by Mahafza, account for uncertainty in the aircraft pose.
This paper presents a framework for incorporating aircraft state uncertainty into the single-pulse radar detection model presented by Mahafza.
The results of this work justify the consideration of aircraft pose uncertainty in the radar detection model as it has a significant impact on the probability of detection.
}
%}% revision

The primary contribution of this paper is a framework for combining aircraft state uncertainty with single-pulse radar detection models to enable enhanced path planning approaches. This is accomplished by linearizing the expression for the probability of detection with respect to aircraft pose. The linearized system is then used to approximate, to the first order, the variance of the probability of detection. The results validate the linearization by running a Monte Carlo analysis and illustrate the sensitivity of the probability of detection to aircraft pose uncertainty. The framework may be used by mission planners to better understand the detection risk, plan more intelligent paths, and make UAV design decisions, such as determining the required sensor quality.

This paper is organized as follows. The single-pulse radar detection and RCS models are discussed in Section \ref{sec:RadarDetectionModel}. The framework for linearizing the expression for the probability of detection and incorporating aircraft pose uncertainty is presented in Section \ref{sec:LinPd}. The results for this paper are provided in Section \ref{sec:Results} where the linearization is validated and the sensitivity of the probability of detection to aircraft pose uncertainty is presented.
